Learning to Limit Data Collection via Scaling Laws: A Computational Interpretation for the Legal Principle of Data Minimization

Modern machine learning systems are increasingly characterized by extensive personal data collection, despite the diminishing returns and increasing societal costs of such practices. Yet, data minimisation is one of the core data protection principles enshrined in the European Union's General Data Protection Regulation ('GDPR') and requires that only personal data that is adequate, relevant and limited to what is necessary is processed. However, the principle has seen limited adoption due to the lack of technical interpretation. In this work, we build on literature in machine learning and law to propose FIDO, a Framework for Inhibiting Data Overcollection. FIDO learns to limit data collection based on an interpretation of data minimization tied to system performance. Concretely, FIDO provides a data collection stopping criterion by iteratively updating an estimate of the performance curve, or the relationship between dataset size and performance, as data is acquired. FIDO estimates the performance curve via a piecewise power law technique that models distinct phases of an algorithm's performance throughout data collection separately. Empirical experiments show that the framework produces accurate performance curves and data collection stopping criteria across datasets and feature acquisition algorithms. We further demonstrate that many other families of curves systematically overestimate the return on additional data. Results and analysis from our investigation offer deeper insights into the relevant considerations when designing a data minimization framework, including the impacts of active feature acquisition on individual users and the feasability of user-specific data minimization. We conclude with practical recommendations for the implementation of data minimization.

==> 04_method.tex <==
% \section{Data Collection Method}
\section{Data Minimization via Scaling Laws}
%\asia{todo: we need a method that models the collection stages accurately but at the same time is as straightforward as possible to enable transparency and audits.}\divya{since this is addressed in the intro; maybe no need here? commenting out for now, but can always add it back in}
The framework accepts three parameters: feature acquisition algorithm $\dmPolicy$, model $\dmModel$, and performance metric $\sigma$.  
There are three steps: (1) $\dmPolicy$ acquires a portion of the available data (\emph{Data Collection}), (2) the performance curve is fit to the new data (\emph{Curve Fitting}), and (3) Steps 1 and 2 repeat until the conditions of Step 3 (\emph{Stopping Criterion Evaluation}) are met.


\subsection{Step 1: Collect Data.} In this step, a feature acquisition algorithm $\dmPolicy$ collects $\dmNumQueries$ observations from the pool of available observations $\dmPool$. Smaller $\dmNumQueries$ translate to more conservative data collection processes and to more accurate estimates of the stopping criterion at the expense of decreased efficiency (smaller $\dmNumQueries$ mean that Steps 2 and 3 are executed more frequently). One might choose to set a larger $\dmNumQueries$ early on during data processing, and decrease it as the data processing continues. 

\subsection{Step 2: Fit the Performance Curve.}
The key idea underpinning this step is to model the stages of data collection \textit{separately} via a piecewise power law curve. The piecewise power law curve is the piece-wise combination of two power law curves \footnote{Modeling the small data region via a third power law curve offered no significant improvement due to its negligible length.}, which we will refer to as $\dmLowerBound$ and $\dmUpperBound$:
%, which we denote $\dmLowerBound$ and $\dmUpperBound$ respectively. 
\begin{equation}
f(x) = \begin{cases} 
      f_0(x) = a_0x^{-b_0} & 0\leq x \leq t \\
      f_1(x) = a_1x^{-b_1} & t \leq x \\
   \end{cases}
\end{equation} 
where $f(x)$ accepts as input a training set size $x$. We fit the piecewise power law curve to subsamples of $\dmHistoricData$ of different sizes. More specifically, given the query size parameter $\dmNumQueries$, we generate \( |\dmHistoricData| / \dmNumQueries\)  samples such that the size of each consecutive sample increases by $q$. We train the model on each sample and evaluate model performance on $\dmValidation$. The resulting pairs of values (sample size and performance on the validation set) are then used to fit $f(x)$. Details on how we fit the parameters are included in the supplement \divya{could include this inline}. 


%We learn these parameters by linearizing the power law equation and applying an ordinary least squares (OLS) method. Past work shows that linearizing the equation produces more stable performance curve estimates \cite{xiao2011use}. 

Finally, we choose a threshold $t$ such that the \emph{slopes} of $\dmLowerBound$  and $\dmUpperBound$ maximally differ. More formally, assuming $b_0^t$ refers to the decay parameter of the first power law curve trained given a threshold  of $t$, we set $t$ to be:
\begin{equation}
    \max_{t \leq |\dmHistoricData|} |b_0^t - b_1^t|
\end{equation}
This follows our intuition regarding the power law region and the diminishing returns region: namely, that the two stages are distinguished by the differing \emph{return} in additional data. Note that in this paper we assume that model performance increases as we collect more data. This is a common assumption in the performance curve literature \cite{kolachina2012prediction, hestness1712deep}, but there are cases in which additional data may hurt model performance. We discuss one such case in Section \ref{sec:user-specific}. In these settings, a different family of parametric curves should be used.  \divya{note how this frameowrk is flexible to different eprformance curve definitions - this paper advances how the piecewise power law curve is appropriate for recommendation systems, but the framework may be appleid iwth different perf curve models in other domains}

In theory, one could compute a stopping criterion directly from the subsamples of $\mathcal{A}$, without fitting the performance curve. This has two undesirable consequences. The first is the instability of the resulting stopping criteria, due to the noise inherent to individual subsamples, as we will see in later experiments. Second, learning a performance curve allows the data minimizer to reason about performance given additional data, \emph{without collecting that data}. This affords the framework flexibility to a range of data minimization objectives, including those that cease data collection based on absolute model performance rather than performance increase rate (relevant experiments are in the supplement).  


% We use the difference in slopes between the power law and diminishing returns region to automatically determine the threshold between the two functions. Concretely, we choose a threshold $t$ such that the We can use our intuition about the difference between these two regions--- the slope of the curve---to automatically determine the threshold between the two functions.


% Validation set performance is measured by the MSE of the FunkSVD \cite{10030079604} reconstruction of rank $r$. \asia{I think this previous sentence should go to the experiments section.} This performance can also be measured through n-fold cross-validation.

% \asia{I think we can skip the above for space.}

% For both $\dmLowerBound$ and $\dmUpperBound$, we assume a power law relationship and learn the parameters $\dmBoundParameterA$ and $\dmBoundParameterB$ for the following equation: 

% \begin{equation}
%     \dmBoundFn(x) = \dmBoundParameterA x^{-\dmBoundParameterB}
% \end{equation}

% We linearize this equation to produce:

% \begin{equation}
%     \log(\dmBoundFn(x)) = -\dmBoundParameterB\log(\dmBoundParameterA) - \dmBoundParameterB\log(x)
% \end{equation}


% Past work shows that linearizing the equation produces more stable performance curve estimates \cite{xiao2011use}. One can fit the learning curve using an ordinary least squares (OLS) method. 

% We choose to train $\dmUpperBound$ on the largest sample sizes because the function is ultimately used to forecast model performance given additional data. This extrapolation is best informed by larger sample sizes, which are more likely to lie in the same data collection phase.

% The choice to train $\dmLowerBound$ to estimate performance given $\dmTraining$ is more subtle. One could use the validation set performance of $\dmModel$ given  $\dmSet{\dmTraining}$. However, this performance is a point estimate of the true value. By training $\dmLowerBound$, we allow our estimate to be informed by sample sizes close to $\dmSetSize{\dmTraining}$, as well.

    

% Validation set performance is measured by the MSE of the FunkSVD \cite{10030079604} reconstruction of rank $r$. \asia{I think this previous sentence should go to the experiments section.} This performance can also be measured through n-fold cross-validation.

\subsection{Step 3: Evaluate Stopping Criteria.} In this step, the resulting performance curve is used to accomplish a specific data minimization objective. Note that these are not the only reasonable data minimization objectives and the framework can adapt to different formulations. 

Minimizing by returns requires the data collector to specify a threshold for return after which data collection should stop, $\dmSlopeThreshold \in \mathbb{R}$. We can use the performance curves to estimate this quantity by taking the derivative at a given sample size: 
\begin{equation}
\dmSlopeEstimate = \begin{cases} 
      -b_0 a_0x^{-b_0-1} & 0\leq x \leq t \\
      -b_1 a_1x^{-b_1-1} & t \leq x \\
   \end{cases}
\end{equation}
Once $\hat{s}$ falls below $\dmSlopeThreshold$, data collection stops.


% \subsubsection{What do these hyperparameters mean?} The query size \textit{q} dictates how often you evaluate your stopping criterion. A larger \textit{q} means you may overshoot your goal percentage, but also means fewer querying steps.

% The sample increment \textit{s} dictates at what interval you sample data to fit the learning curve. Smaller \textit{s} correspond to evaluating more increments of the data and is more computationally expensive.

% The rank \textit{r} refers to the underlying complexity of the matrix you're trying to reconstruct (and I use 30 because other papers have).

==> 98_01_alternate_slope_table.tex <==
\begin{table*}
\centering
%\caption{\textbf{Performance over diminishing return criterion.} Each value is the fraction of data collected using different methods to adhere to a threshold on return (MSE per additional feature-value). Our method halts data collection closest to the true stopping point for a given threshold.}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l|c|ccccccc}
\toprule
      Dataset & Threshold & 2P-PL-Initial &         2P-PL &         3P-PL &     3P-PL-Exp &         Naive &          Ours &          True \\
\midrule
GoogleLocal-L &  -5.0e-07 & $0.32 \pm 0.00$ & $0.32 \pm 0.01$ & $0.32 \pm 0.01$ & $0.16 \pm 0.00$ & $0.27 \pm 0.02$ & $0.29 \pm 0.02$ & $0.27 \pm 0.01$ \\
GoogleLocal-L &  -2.0e-07 & $0.73 \pm 0.01$ & $0.61 \pm 0.01$ & $0.53 \pm 0.01$ & $0.25 \pm 0.01$ & $0.36 \pm 0.04$ & $0.42 \pm 0.03$ & $0.40 \pm 0.03$ \\
GoogleLocal-L &  -5.0e-08 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $0.40 \pm 0.02$ & $0.52 \pm 0.08$ & $0.65 \pm 0.04$ & $0.64 \pm 0.04$ \\
GoogleLocal-S &  -5.0e-07 & $0.88 \pm 0.01$ & $0.71 \pm 0.01$ & $0.60 \pm 0.01$ & $0.28 \pm 0.01$ & $0.37 \pm 0.07$ & $0.42 \pm 0.06$ & $0.42 \pm 0.07$ \\
GoogleLocal-S &  -2.0e-07 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $0.91 \pm 0.03$ & $0.39 \pm 0.01$ & $0.44 \pm 0.08$ & $0.48 \pm 0.09$ & $0.46 \pm 0.09$ \\
GoogleLocal-S &  -5.0e-08 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $0.55 \pm 0.01$ & $0.46 \pm 0.09$ & $0.56 \pm 0.04$ & $0.54 \pm 0.04$ \\
  MovieLens-L &  -5.0e-07 & $0.13 \pm 0.00$ & $0.13 \pm 0.00$ & $0.13 \pm 0.00$ & $0.13 \pm 0.00$ & $0.14 \pm 0.01$ & $0.13 \pm 0.00$ & $0.13 \pm 0.00$ \\
  MovieLens-L &  -2.0e-07 & $0.29 \pm 0.00$ & $0.27 \pm 0.00$ & $0.26 \pm 0.00$ & $0.13 \pm 0.00$ & $0.25 \pm 0.01$ & $0.24 \pm 0.01$ & $0.24 \pm 0.01$ \\
  MovieLens-L &  -5.0e-08 & $1.00 \pm 0.00$ & $0.76 \pm 0.01$ & $0.62 \pm 0.01$ & $0.24 \pm 0.01$ & $0.43 \pm 0.08$ & $0.52 \pm 0.05$ & $0.53 \pm 0.03$ \\
  MovieLens-S &  -5.0e-07 & $0.50 \pm 0.02$ & $0.53 \pm 0.01$ & $0.51 \pm 0.01$ & $0.23 \pm 0.01$ & $0.37 \pm 0.04$ & $0.46 \pm 0.05$ & $0.45 \pm 0.02$ \\
  MovieLens-S &  -2.0e-07 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $0.97 \pm 0.02$ & $0.36 \pm 0.01$ & $0.51 \pm 0.08$ & $0.67 \pm 0.12$ & $0.68 \pm 0.10$ \\
  MovieLens-S &  -5.0e-08 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $0.64 \pm 0.02$ & $0.66 \pm 0.22$ & $0.97 \pm 0.07$ & $0.97 \pm 0.08$ \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Accuracy of Data Collection Stopping Point.} We compare each of the baselines to an alternate approximation of the true slope here. Instead, we calculate the slope over two  adjacent subsamples rather than four. We see that the piecewise power law curve adheres most closely to the empiricaly derived true stopping point.}
\label{diminishing_returns_table_different_approx}
\end{table*}

==> 98_02_stage_ablations.tex <==
\begin{table*}
\centering
%\caption{\textbf{Performance over diminishing return criterion.} Each value is the fraction of data collected using different methods to adhere to a threshold on return (MSE per additional feature-value). Our method halts data collection closest to the true stopping point for a given threshold.}
\resizebox{.6\textwidth}{!}{%
\begin{tabular}{l|c|cccccc|c}
\toprule
      Dataset & Threshold & FIDO (1 Stage) & FIDO (2 Stages) & FIDO (3 Stages) &        Oracle \\
\midrule
GoogleLocal-L &  -5.0e-07 &  $0.32 \pm 0.01$ &   $0.29 \pm 0.02$ &   $0.29 \pm 0.02$ & $0.27 \pm 0.01$ \\
GoogleLocal-L &  -2.0e-07 &  $0.61 \pm 0.01$ &   $0.42 \pm 0.03$ &   $0.42 \pm 0.03$ & $0.41 \pm 0.02$ \\
GoogleLocal-L &  -5.0e-08 &  $1.00 \pm 0.00$ &   $0.65 \pm 0.04$ &   $0.68 \pm 0.05$ & $0.68 \pm 0.05$ \\
GoogleLocal-S &  -5.0e-07 &  $0.71 \pm 0.01$ &   $0.42 \pm 0.06$ &   $0.42 \pm 0.06$ & $0.47 \pm 0.03$ \\
GoogleLocal-S &  -2.0e-07 &  $1.00 \pm 0.00$ &   $0.48 \pm 0.09$ &   $0.51 \pm 0.14$ & $0.58 \pm 0.06$ \\
GoogleLocal-S &  -5.0e-08 &  $1.00 \pm 0.00$ &   $0.56 \pm 0.04$ &   $0.59 \pm 0.08$ & $0.64 \pm 0.10$ \\
  MovieLens-L &  -5.0e-07 &  $0.13 \pm 0.00$ &   $0.13 \pm 0.00$ &   $0.13 \pm 0.00$ & $0.13 \pm 0.00$ \\
  MovieLens-L &  -2.0e-07 &  $0.27 \pm 0.00$ &   $0.24 \pm 0.01$ &   $0.25 \pm 0.02$ & $0.23 \pm 0.01$ \\
  MovieLens-L &  -5.0e-08 &  $0.76 \pm 0.01$ &   $0.52 \pm 0.05$ &   $0.53 \pm 0.05$ & $0.53 \pm 0.02$ \\
  MovieLens-S &  -5.0e-07 &  $0.53 \pm 0.01$ &   $0.46 \pm 0.05$ &   $0.46 \pm 0.05$ & $0.45 \pm 0.03$ \\
  MovieLens-S &  -2.0e-07 &  $1.00 \pm 0.00$ &   $0.67 \pm 0.12$ &   $0.68 \pm 0.14$ & $0.79 \pm 0.08$ \\
  MovieLens-S &  -5.0e-08 &  $1.00 \pm 0.00$ &   $0.97 \pm 0.07$ &   $0.99 \pm 0.03$ & $1.00 \pm 0.00$ \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Ablation of the Number of Stages in FIDO's Performance Curve Model.} We vary the number of stages we assume to exist in the performance curve between 1 (assuming the entire performance curve can be described by a power law) and 3 (aligning with the number of stages described by \cite{hestness1712deep}. FIDO achieves the closest stopping criterion (on average) to Oracle when the framework models three stages of data collection.}
\label{diminishing_returns_ablation_table}
\end{table*}

==> 98_03_nonparam_comparison.tex <==
\begin{table*}
\centering
%\caption{\textbf{Performance over diminishing return criterion.} Each value is the fraction of data collected using different methods to adhere to a threshold on return (MSE per additional feature-value). Our method halts data collection closest to the true stopping point for a given threshold.}
\resizebox{.5\textwidth}{!}{%
\begin{tabular}{l|c|cccccc|c}
\toprule
      Dataset & Threshold &      NonParam &          FIDO &        Oracle \\
\midrule
GoogleLocal-L &  -5.0e-07 & $0.28 \pm 0.01$ & $0.29 \pm 0.02$ & $0.27 \pm 0.01$ \\
GoogleLocal-L &  -2.0e-07 & $0.30 \pm 0.01$ & $0.42 \pm 0.03$ & $0.41 \pm 0.02$ \\
GoogleLocal-L &  -5.0e-08 & $0.30 \pm 0.01$ & $0.68 \pm 0.05$ & $0.68 \pm 0.05$ \\
GoogleLocal-S &  -5.0e-07 & $0.32 \pm 0.01$ & $0.42 \pm 0.06$ & $0.47 \pm 0.03$ \\
GoogleLocal-S &  -2.0e-07 & $0.32 \pm 0.01$ & $0.51 \pm 0.14$ & $0.58 \pm 0.06$ \\
GoogleLocal-S &  -5.0e-08 & $0.32 \pm 0.02$ & $0.59 \pm 0.08$ & $0.64 \pm 0.10$ \\
  MovieLens-L &  -5.0e-07 & $0.15 \pm 0.01$ & $0.13 \pm 0.00$ & $0.13 \pm 0.00$ \\
  MovieLens-L &  -2.0e-07 & $0.25 \pm 0.01$ & $0.25 \pm 0.02$ & $0.23 \pm 0.01$ \\
  MovieLens-L &  -5.0e-08 & $0.28 \pm 0.01$ & $0.53 \pm 0.05$ & $0.53 \pm 0.02$ \\
  MovieLens-S &  -5.0e-07 & $0.39 \pm 0.01$ & $0.46 \pm 0.05$ & $0.45 \pm 0.03$ \\
  MovieLens-S &  -2.0e-07 & $0.39 \pm 0.01$ & $0.68 \pm 0.14$ & $0.79 \pm 0.08$ \\
  MovieLens-S &  -5.0e-08 & $0.39 \pm 0.01$ & $0.99 \pm 0.03$ & $1.00 \pm 0.00$ \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Comparison of FIDO to non-parametric regression.} FIDO achieves more accurate stopping criteria than nonparametric regression across datasets and thresholds.}
\label{nonparam_table}
\end{table*}

==> deprecated/02_problem_statement.tex <==


\section{Background: GDPR's Data Minimization}

The GDPR requires that no more data than is necessary to achieve a declared \emph{processing purpose} (in line with the purpose limitation principle) be processed. Data minimization is both a key principle under Article 5(1)(c) GDPR as well as a component of data protection by design and by default.

While it has been shown empirically that data can be minimized through various domain- and algorithm-specific heuristics~\cite{biega2020dm}, a question remains of how to automatically learn when to stop data collection for various personalization systems and feature acquisition strategies; the remainder of this paper focuses on this problem. In particular, we focus on \emph{depth-based} data, which concerns the volume of data collected. For a thorough treatment of the harms data minimization protects against, we refer the interested reader to \citet{finckreviving}.

% \subsection{Example Scenarios and Harms}
% \asia{It might actually make sense to move this after 3.1}
% This interpretation applies broadly to different profiling and decision making systems, including recommendation and classification. We highlight three examples to ground our contributions:

% \begin{itemize}
%     \item A recommender system collects movie ratings to provide personalized movie recommendations. The systems might not need all user rating data but is able to provide recommendations with only a minor error increase using ratings from only the most recent 6 months. 
%     \item An algorithm collects \emph{likes} for gastronomy pages to provide restaurant advertisements. It might deliver near optimal results by storing only a single \emph{like} for each cuisine category for each user. 
%     \item ...
% \end{itemize}


\subsection{Computational and Legal Basis}

The key proposal in this paper is to maximally limit data collection given a target performance using \emph{performance curves}. We contrast the true performance curve for the GoogleLocal-L dataset \cite{pasricha2018translation} with a figure from \citet{hestness1712deep} that identifies three phases of data collection (Fig. \ref{perf_curves}). The phases are:

\begin{enumerate}
    \item \emph{The small data region}, where the collected data is insufficiently representative and model performance is poor.
    \item \emph{The power-law region}, where there is a direct trade-off between the amount of data collected and performance.
    \item \emph{The irreducible error region}, where the collection of more data does not lead to model improvements.
\end{enumerate}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{LaTeX/figs/two_performance_curves.png}
        \vspace{-0.6cm}
    \caption{\footnotesize Model performance over the course of data collection. On the left, a figure from \citet{hestness1712deep} plots the phases of data collection. On the right, we plot model performance over data collection from GoogleLocal. Preprocessing details can be found in the supplement.}
    \label{perf_curves}
    \vspace{-0.5cm}
\end{figure}




% Figure \ref{perf_curves} includes the relationship for GoogleLocal-S (a 500 user sample of GoogleLocal) and GoogleLocal-L (a 5000 user sample of GoogleLocal). Preprocessing details for each dataset can be found in the Experimental Set-Up section. 
    
%     We make two observations from Figure \ref{perf_curves}. The first is that the stages of data collection identified by \citet{hestness1712deep} in machine translation exist for recommendation dat asets. This is true for both the small and large sample of GoogleLocal. We include preprocessing details for the dataset in the Experimental Set-Up section.
    
%     The second observation is that a mere 10\% of the dataset lands data collection outside of the small data region.  
% A majority of data collection occurs between the power law region and the diminishing returns region. This has important implications for modeling the performance curve. Modeling the entire region using the power law curve produces underestimates when predicting error given additional data. In later sections, we show that modeling each stage separately mitigates this effect.

From a practical perspective, the data collection phases could be used to decide when collecting more data is necessary for reliable model performance (the small data region), when a user should decide whether to trade more data for better performance (the power-law region), and when data collection should stop (the irreducible error region).

The distinction of these phases is also pertinent from a legal perspective. In particular, the application of data minimization's necessity criterion would indicate that continued collection of personal data in the third phase would be hard to justify as it is not ``necessary" to improve the model and meet its underlying purpose. We formalize these implications into a formal stopping criterion based on an empirical derivative of the the learned performance curve.
% two objectives in the following section: halting data collection after 1) achieving a pre-specified fraction of performance gain, or 2) falling below a pre-specified threshold for return on additional data.


% \asia{The notation needs to be described in more detail so that it's clear what H(D, n) is returning, and what signature datasets have.}

\subsection{Formal Interpretation}
% Data minimization must be operationalized with respect to a specific data processing \emph{purpose}. 
% We build on the approach put forward by \citet{biega2020dm} in which the processing purpose is associated with \emph{improvements in model performance metrics}. 
We follow a recent interpretation that ties data collection to \emph{model performance metrics}~\cite{biega2020dm}. For example, models meant for clinical deployment may require a sufficient amount of data to be deemed safe for public use. This is similar to the way clinical studies estimate the sample size required to meet a significance threshold, but notably limit sample sizes to avoid distributing an untested treatment to an unnecessarily large population \cite{gupta2016basic}.

However, operationalizing this interpretation remains unclear. We propose a formalization based on the returns in performance from additional data.

\subsubsection{Scenario and Notation.} We assume a scenario where a data processor operates a service (a model $\dmModel$, such as a recommender system) and collects data from a pool of queryable data $\dmPool$ (consisting of user-feature-value triples) generated by a population of users $\dmUsers$.  We define $\dmModel$ as the collection of parameters learned using personal data, including hyperparameters. There is an implicit relationship between model complexity and the amount of data required to achieve a specific performance. While we assume a fixed model, one may apply this framework to multiple models and select the model which requires the least data. 

The acquired data is used to train $\dmModel$ and make predictions for each user $\dmUser \in \dmUsers$. We further assume that, when the data collection starts, the data processor has access to some initial data: $\dmTraining$ for training the model and $\dmValidation$ set aside to validate model performance predictions. Such initial data would include any data that is historical, purchased, or collected in different markets.

During data collection, the processor applies a feature acquisition policy $\dmPolicy(\dmPool, \dmBudget)$ which queries $n$ feature values from $\dmPool$.  Queries equate to the collection of a specific user-feature-value for inclusion in the training set for model $\dmModel$. We refer to the union of initial and acquired data as $\dmHistoricData$ and let $|\cdot|$ denote the cardinality of a set. Let $\dmPerformance$ represent the true performance curve for $\dmModel$, which maps a domain of training dataset sizes to a range of model performances as measured by a performance metric $\sigma$. User-specific performance curves for $\dmModel$ are termed $\dmUserPerformance$ for a given user $\dmUser$. The objective used to train $\dmModel$ translates to the processing purpose.

The processor can use the resulting predicted performance curve to adhere to a concrete data minimization objective. We propose one such objective below: \emph{returns-based} data minimization. 

\subsubsection{Minimizing by Returns in Performance.}  We minimize in reference to a threshold on the \textit{return} in model performance of additional data. One could select an appropriate threshold by assessing user preferences or selecting a  sufficiently small threshold such that user experience is not affected. Formally, a data collector would cease data collection once the slope of the performance curve drops below threshold $t$: 
%One may instead wish to limit the collection of data when the return to model performance falls below a certain threshold.
\begin{equation}
    \frac{d\dmPerformance}{dn}(|\mathcal{A}|) \leq t
\end{equation}
Producing an accurate approximation of $\dmPerformance$ is thus central to any performance-based data minimization objective. Our experiments show that existing approaches produce performance curves that are insufficient for the stated objectives. We compensate for these shortcomings by proposing a more accurate method to approximate $\dmPerformance$.
%
Experiments in the supplement furthermore engage an alternate formalization of data minimization, where the stopping criterion is determined by the \emph{relative model performance} achieved rather than the performance returns, providing further evidence of the framework's flexibility.

% access to initial data $\mathcal{I}$, validation data $\mathcal{V}$ and a pool of queryable data $\mathcal{P}$. The interpretation is flexible to the following user-specified parameters:

% \begin{itemize}
%     \item $M$: Model $M$ refers to the model intended for training on the acquired data.
%     \item $H(D, n)$: Feature acquisition algorithm $H$ queries $n$ feature values from dataset $D$. 
%     \item $\sigma(M, D)$: Performance metric $\sigma$ measures the performance of model $M$ trained on dataset $D$ on a held-out test set.
%     \item $g$: Percentage of performance gain $g$ refers to the goal percentage of performance gain. This parameter dictates when the stopping criterion is enforced.
% \end{itemize}




%\paragraph{Comments and intuitions:}
%Minimizing in reference to a relative performance rather than an absolute performance allows us to account for two factors---the performance contributions of the initialization data (data already existing in the system---historical, purchased, collected from other markets, etc.), as well as the irreducible model error. Irreducible model error describes the fact that the diminishing returns for additional data rarely occur at a classification performance of 100\% or an MSE of 0. It is difficult to identify a good goal performance without understanding (1) model performance in the absence of additional data and (2) model performance in the presence of all available data.
 


%\divya{Sentence about how predicting BPP is a forecasting task, while predicting current and initial performance are easier}.


==> deprecated/12_conclusion.tex <==
\section{Discussion}
The adoption of the GDPR's data minimization principle has been hindered a dearth of computational formalizations~\cite{finckreviving}.
Aligning insights and concepts in machine learning and law, this paper offers the first interpretation connecting data minimization with learning performance curves, developing formal minimization objectives and a framework that learns appropriate data collection stopping points. 
%
Our empirical investigation offers guidance on the implementation of data minimization. We demonstrated how active feature acquisition--a technique which might be thought of as a go-to tool for data minimization--can be undesirable in the context of personal data protection. We found that AFA might place excess data collection burden on a small set of users, and that the technique's performance depends on data initialization conditions, with degrading performance in simulations of evolving user communities or restricted feature sets.

In light of these complexities, we believe that data minimization compliance in machine learning models will require similar efforts as the principle of fairness has garnered. Definitions, formal implementations and caveats will depend on the application domain, the underlying model (recommendation, classification)
%, as well as societal, cultural and individual preferences (when to minimize, or which data to prioritize). 
The piecewise power law may not be appropriate for all domains, including user-specific data minimization.
%and cases where additional data significantly degrades model performance. 
Moreover, adversarial approaches are possible: a data processor acting in bad faith may choose a model class that requires a large amount of personal data. Further research is necessary to ensure data minimization occurs despite malicious data collection practices.

Finally, it is important to recognize that GDPR does not impose a hierarchy of importance of different principles -- data minimization and other principles must be satisfied at the same time. In practice, this requires examining the trade-offs between different data protection principles. While this paper focuses on the relationship between data minimization and accuracy, our empirical study, like some of the prior work~\cite{finckreviving,biega2020dm,galdon2020auditing}, suggests there exists a tension between data minimization and fairness. Reconciling such tensions and making sure data minimization does not disproportionately affect marginalized populations will be imperative to broader adoption.

% \paragraph{Choosing a Feature Acquisition Algorithm} Based on our experiments, we recommend random feature acquisition to guide data minimization. We base this recommendation on three reasons: 1) random feature acquisition produces a smoother performance curve, and thus, more accurate performance estimates, 2) our work confirms recent findings that demonstrate how the success of intelligent data collection depends upon initialization conditions \cite{munjal2020towards}, and 3) AFA algorithms can place excess data collection burden on specific users, as our user-specific impact analyses show. We explore the possibility of combining AFA and random feature acquisition in the supplement.

%\noindent\textbf{Choosing a Performance Curve Model} The piecewise power law curve model is best fit to describe the relationship between dataset size and performance. We see that this choice may not be consequential when the diminishing returns region is small, as is the case with MovieLens-S.

%\paragraph{Creating a Representative Validation Set} This framework hinges on the creation of a representative validation set. As is the case with many systems that operate on continuously collected data, a representative validation set may need to be recreated to account for  temporal shift. \divya{rephrase or replace with query size}

%\paragraph{Identifying a Relevant Objective.} While the framework we propose is flexible to many objectives, it is worth considering when one objective may be more desirable than another. One can consider its \emph{ease of definition}: how well does the selected objective reflect user preferences? Between the objectives we propose, gauging user preferences in terms of relative performance may be easier to survey for than diminishing returns. One could also consider the objective's \emph{specificity}. Experiments in the supplement show that minimizing by diminishing returns is more accurate earlier on during data collection compared to minimization by relative performance.  %Dataset size plays a role too, as our experiments show that both the prediction of returns and relative performance are noisier in smaller datasets. 

%When/why would you use a performance-based  stopping criterion? Ease of definition, easier to define for higher percentages, easier to define for smaller datasets.

%When/why would you want to use a diminishing returns based criterion? More accurate for goals that lie in the power law region (we see that the performance-based stopping criterion is more difficult to adhere to at lower percentages, whereas the accuracy of the slope prediction is more accurate). 

% \newline
% \noindent\textbf{Performing User-Specific Impact Analyses.} Data minimization may disproportionately affect marginalized populations. Recent work \cite{tae2020slice, chen2018my} has shown that in some instances, it is necessary to  collect \emph{more} data to ensure the equitable performance. As a result, it is imperative to perform per-user analyses when studying and proposing methods for data minimization.  

% While our paper provides new methods, insights and practical guidelines for implementing data minimization in automated personalization and profiling systems, several open questions remain. Those include, for instance, designing more accurate per-user minimization methods, automatic detection of data collection stages, and studying the technical interplay between data minimization and other data protection principles. Moreover, adversarial approaches are possible: a data processor acting in bad faith may choose a model class that requires a large amount of personal data. Further research is necessary to ensure data minimization occurs despite malicious data collection practices.



%\section{Discussion}
%\label{conclusion}


%This work aims to bridge the gap between the legal principle of data minimization and its practical realization. Data-driven systems often operate under the assumption that more data is unequivocally better, for all parties involved. This might not the case when the identifiability, sensitivity, liability, and storage costs of collected data are acknowledged and appropriately balanced. We intend our work to be a step towards respectful data collection. Our findings offer takeaways for practitioners, legal scholars, and researchers. 

%Concretely, we make three contributions: 1) a framework for data minimization that advances existing approaches to performance curve modeling, 2) a close analysis of the proposed framework's performance on two data minimization objectives that sheds light on the relevant considerations when designing a data minimization approach and 3) a synthesis of practical recommendations for the implementation of data minimization. \divya{clean this up}

%We propose a method for data minimization during data collection that relies on adaptively learning the relationship between dataset size and performance and accounts for three distinct stages of data collection. Each data collection stage is characterized by quantitatively different contributions to system performance, with the second stage allowing users to trade data for improved performance, and the last stage characterized by no significant performance increase and thus offering a definite stopping point. Moreover, we find that the quantitative changes between data collection phases cause existing approaches to overestimate the amount of data necessary to meet a target performance. We also demonstrate that AFA methods may incur unequal distribution of collected data across users, and decreased performance for evolving communities or in cases where certain features are excluded from initial data collection. \divya{thought for later: remove this paragraph? combine content with beginning of Section 9?}

%While our paper provides new methods, insights and practical guidelines for implementing data minimization in automated personalization and profiling systems, several open questions remain. Those include, for instance, designing more accurate per-user minimization methods, automatic detection of data collection stages, and studying the technical interplay between data minimization and other data protection principles.
 
% We show that the proposed approach is more accurate in terms of predicting model performance metrics than existing approaches across datasets, feature acquisition algorithms, and data initialization assumptions.
%
% Promising directions for future work follow naturally from our experiments, including improving the accuracy of user-specific performance curves and mitigating the impact of active feature acquisition on data subjects. We describe the importance of these findings to legal scholars, data processors, and researchers below.
%
% \subsubsection{Legal scholars.}  Our work highlights three distinct stages of data collection, each with quantitatively different contributions of new data to the system performance. We moreover show the over-collection of data using a performance-based stopping criterion, and the impact of active feature acquisition on data subjects. We intend our work to serve as a foundation for detailed, task-specific legal specifications for data minimization.

%Experiments demonstrate the flexibility of our interpretation to technical choices, including initialization assumptions and feature acquisition algorithms. 

% \subsubsection{Data processors.} We provide the first method designed for data minimization during data collection. Experiments in the paper confirm the existence of three stages of data collection and present the implications of these phases for data processors. We intend these experiments to illuminate the role global and user performance curves can play in understanding the data collection process. 
% We make our code publicly available as a resource for implementing data minimization. 

% \subsubsection{Researchers.} We show that an assumption made by existing approaches to learning performance curves---namely, the use of a single power law relationship---does not hold in the context of recommendation. We show that modeling stages of data collection separately allows our method to outperform existing approaches across datasets, feature acquisition algorithms, and initialization assumptions. Open questions include automatically identifying the transition from the power-law region to the diminishing returns region and understanding the prevalence and span of the diminishing returns region across a broader set of tasks. 
 
 %We identified a systematic weakness of existing approaches to learning performance curves. Namely, existing approaches assume a power law relationship throughout data collection.

==> deprecated/to_delete.tex <==
\section{Experimental Details}

We include relevant details to our experimentation below and provide code to reproduce all results.

\paragraph{Dataset Pre-Processing} For MovieLens-20M, we filter out users with fewer than 100 movies rated to produce a dataset of 51869 users and 26654 unique movies. MovieLens-L randomly samples 5000 users from this set and MovieLens-S samples 1000 users. For GoogleLocal, we filter out users with fewer than 150 ratings to produce a dataset of 1571 users and 275402 unique places. GoogleLocal-L randomly samples 1500 users from this set and GoogleLocal-S samples 500 users. Table 1 summarizes the dimensionality and sparsity of the resulting datasets.

\paragraph{Parameter Fitting} In line with past work, our method and each baseline is subject to the same parameter fitting approach: weighted non-linear least squares (NLSw). NLSw weights each sample by $( 1/\sqrt n)$, where $n$ is the sample size. This is done to account for the heteroscedastic relationship between performance  and dataset size. 

\paragraph{Hyperparameters} We assume the model $\dmModel$ operated by the data processor is a FunkSVD \cite{funk2006netflix} recommendation system. We use the same hyperparameters $r$ and $\dmNumQueries$ across all experiments: the number of latent  features in FunkSVD is set to be 30, and $\dmNumQueries$ is set to be 2\% of the number of queryable entries. We assume random feature acquisition unless otherwise stated. 

\paragraph{Implementation}  We fit performance curves using the OLS implementation included in the Python statsmodels library \cite{seabold2010statsmodels} and the Levenberg-Marquardt algorithm via the least-squares implementation in the Python sklearn library \cite{scikit-learn}. All experiments were run on a 2.8 GHz Intel Core i7 processor with 16GB of available RAM on MacOS High Sierra.

\paragraph{Evaluation} We evaluate each method at three thresholds for the return on additional data: 5e-7, 2e-7, and 5e-8.  We select these thresholds because they translate to thresholds that are distributed over the data collection process (see Figure \ref{diminishing_returns_fig} to observe typical range of empirical returns for MovieLens-L and GoogleLocal-L). 

To make our calculation of the true slope explicit, recall that we  generate $|\dmHistoricData|/\dmNumQueries$ subsamples over the course of data collection. To estimate the return in MSE at subsample $i$, we divide the difference in empirical performance at subsample $i-2$ and subsample $i+2$ by their difference in sample sizes, or $4\dmNumQueries$. This produces an approximation of the true return that is sufficiently smooth; we experiment with a different smoothing procedure (estimation via subsample $i-1$ and subsample $i+1$) later in the supplemental material.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
